Evolution of spin freezing transition and structural, magnetic phase diagram of Dy$_{2-x}$La$_x$Zr$_2$O$_7$; $x$ = 0-2.0

Dy$_{2}$Zr$_{2}$O$_{7}$ a disordered pyrochlore system, exhibits the spin ice freezing under the application of magnetic field. Our studies suggest the stabilization of pyrochlore phase in Dy$_{2-x}$La$_{x}$Zr$_{2}$O$_{7}$ with the substitution of nonmagnetic La, along with the biphasic mixture for the intermediate compositions. We observed that the higher La compositions (1.5 $\leq$ x $\leq$ 1.9), show spin freezing (T $\sim$ 17 K) similar to the field induced spin ice freezing for low La compositions (0 $\leq$ x $\leq$ 0.5), and the well known spin ice systems Dy$_{2}$Ti$_{2}$O$_{7}$ and Ho$_{2}$Ti$_{2}$O$_{7}$. The low temperature magnetic state for higher La compositions (1.5 $\leq$ x $\leq$ 1.9) culminates into spin glass state below 6 K. The Cole-Cole plot and Casimir-du Pr$\acute{e}$ fit shows narrow distribution of spin relaxation time in these compounds.

==> Ref.tex <==
@article{ramon2019absence,
	title={Absence of spin-ice state in the disordered fluorite D y 2 Z r 2 O 7},
	author={Ramon, Jonathan Gustavo Acosta and Wang, CW and Ishida, L and Bernardo, PL and Leite, MM and Vichi, Fl{\'a}vio Maron and Gardner, JS and Freitas, RS},
	journal={Physical Review B},
	volume={99},
	number={21},
	pages={214442},
	year={2019},
	publisher={APS}
}

@article{snyder2003quantum,
	title={Quantum-Classical Reentrant Relaxation Crossover in D y 2 T i 2 O 7 Spin Ice},
	author={Snyder, J and Ueland, BG and Slusky, JS and Karunadasa, H and Cava, Robert Joseph and Mizel, Ari and Schiffer, P},
	journal={Physical review letters},
	volume={91},
	number={10},
	pages={107201},
	year={2003},
	publisher={APS}
}

@article{mandal2006preparation,
	title={Preparation, XRD and Raman spectroscopic studies on new compounds RE2Hf2O7 (RE= Dy, Ho, Er, Tm, Lu, Y): Pyrochlores or defect-fluorite?},
	author={Mandal, BP and Garg, Nandini and Sharma, Surinder M and Tyagi, AK},
	journal={Journal of Solid State Chemistry},
	volume={179},
	number={7},
	pages={1990--1994},
	year={2006},
	publisher={Elsevier}
}

@article{sayed2011sm2,
	title={Sm2- x Dy x Zr2O7 Pyrochlores: Probing Order- Disorder Dynamics and Multifunctionality},
	author={Sayed, Farheen N and Grover, V and Bhattacharyya, K and Jain, D and Arya, A and Pillai, CGS and Tyagi, AK},
	journal={Inorganic chemistry},
	volume={50},
	number={6},
	pages={2354--2365},
	year={2011},
	publisher={ACS Publications}
}

@article{glerup2001structural,
	title={The structural transformation from the pyrochlore structure, A2B2O7, to the fluorite structure, AO2, studied by Raman spectroscopy and defect chemistry modeling},
	author={Glerup, Marianne and Nielsen, Ole Faurskov and Poulsen, Finn Willy},
	journal={Journal of Solid State Chemistry},
	volume={160},
	number={1},
	pages={25--32},
	year={2001},
	publisher={Elsevier}
}

@article{anand2015investigations,
	title={Investigations of the effect of nonmagnetic Ca substitution for magnetic Dy on spin-freezing in Dy2Ti2O7},
	author={Anand, VK and Tennant, DA and Lake, B},
	journal={Journal of Physics: Condensed Matter},
	volume={27},
	number={43},
	pages={436001},
	year={2015},
	publisher={IOP Publishing}
}

@article{snyder2001spin,
	title={How ‘spin ice’freezes},
	author={Snyder, J and Slusky, JS and Cava, Robert Joseph and Schiffer, P},
	journal={Nature},
	volume={413},
	number={6851},
	pages={48},
	year={2001},
	publisher={Nature Publishing Group}
}

@article{pal2018high,
	title={High temperature spin-freezing transition in pyrochlore Eu2Ti2O7: A new observation from ac-susceptibility},
	author={Pal, Arkadeb and Singh, Abhishek and Ghosh, AK and Chatterjee, Sandip},
	journal={Journal of Magnetism and Magnetic Materials},
	volume={462},
	pages={1--7},
	year={2018},
	publisher={Elsevier}
}

@article{kumar2019spin,
	title={Spin-phonon coupling in hole-doped pyrochlore iridates Y2Ir1-xRux2O7: A Raman scattering study},
	author={Kumar, Harish and Sathe, VG and Pramanik, AK},
	journal={Journal of Magnetism and Magnetic Materials},
	volume={478},
	pages={148--154},
	year={2019},
	publisher={Elsevier}
}

@article{han2015electron,
	title={Electron paramagnetic resonance study of the f--d interaction in pyrochlore iridate Gd2Ir2O7},
	author={Han, Hui and Zhang, Lei and Liu, Hui and Ling, Langsheng and Tong, Wei and Zou, Youming and Ge, Min and Fan, Jiyu and Zhang, Changjin and Pi, Li and others},
	journal={Philosophical Magazine},
	volume={95},
	number={27},
	pages={3014--3022},
	year={2015},
	publisher={Taylor \& Francis}
}
@inproceedings{hasegawa2010raman,
	title={Raman scattering study in iridium pyrochlore oxides},
	author={Hasegawa, T and Ogita, N and Matsuhira, K and Takagi, S and Wakeshima, M and Hinatsu, Y and Udagawa, M},
	booktitle={Journal of Physics: Conference Series},
	volume={200},
	number={1},
	pages={012054},
	year={2010},
	organization={IOP Publishing}
}

@article{hozoi2014longer,
	title={Longer-range lattice anisotropy strongly competing with spin-orbit interactions in pyrochlore iridates},
	author={Hozoi, L and Gretarsson, H and Clancy, JP and Jeon, B-G and Lee, B and Kim, KH and Yushankhai, V and Fulde, Peter and Casa, D and Gog, T and others},
	journal={Physical Review B},
	volume={89},
	number={11},
	pages={115111},
	year={2014},
	publisher={APS}
}

@article{vandenborre1983rare,
	title={Rare-earth titanates and stannates of pyrochlore structure; vibrational spectra and force fields},
	author={Vandenborre, MT and Husson, E and Chatry, JP and Michel, D},
	journal={Journal of Raman Spectroscopy},
	volume={14},
	number={2},
	pages={63--71},
	year={1983},
	publisher={Wiley Online Library}
}

@article{turner2017lanthanide,
	title={Lanthanide stannate pyrochlores (Ln2Sn2O7; Ln= Nd, Gd, Er) at high pressure},
	author={Turner, Katlyn M and Tracy, Cameron L and Mao, Wendy L and Ewing, Rodney C},
	journal={Journal of Physics: Condensed Matter},
	volume={29},
	number={50},
	pages={504005},
	year={2017},
	publisher={IOP Publishing}
}

@article{mydosh1993spin,
	title={Spin Glasses: An Experimental Introduction, Taylor and Francis London},
	author={Mydosh, JA},
	journal={Washington DC},
	year={1993}
}

@article{anand2011signatures,
	title={Signatures of spin-glass behavior in the induced magnetic moment system PrRuSi 3},
	author={Anand, VK and Adroja, DT and Hillier, AD and Taylor, J and Andr{\'e}, G},
	journal={Physical Review B},
	volume={84},
	number={6},
	pages={064440},
	year={2011},
	publisher={APS}
}

@article{bovo2018special,
	title={Special temperatures in frustrated ferromagnets},
	author={Bovo, L and Twengstr{\"o}m, Mikael and Petrenko, OA and Fennell, T and Gingras, MJP and Bramwell, ST and Henelius, Patrik},
	journal={Nature communications},
	volume={9},
	number={1},
	pages={1--8},
	year={2018},
	publisher={Nature Publishing Group}
}

@article{faak2012kapellasite,
	title={Kapellasite: A kagome quantum spin liquid with competing interactions},
	author={F{\aa}k, B and Kermarrec, E and Messio, L and Bernu, B and Lhuillier, C and Bert, F and Mendels, P and Koteswararao, B and Bouquet, F and Ollivier, J and others},
	journal={Physical review letters},
	volume={109},
	number={3},
	pages={037208},
	year={2012},
	publisher={APS}
}

@article{lhotel2015fluctuations,
	title={Fluctuations and All-In--All-Out Ordering in Dipole-Octupole Nd 2 Zr 2 O 7},
	author={Lhotel, Elsa and Petit, Sylvain and Guitteny, Solene and Florea, O and Hatnean, M Ciomaga and Colin, Claire and Ressouche, Eric and Lees, MR and Balakrishnan, G},
	journal={Physical review letters},
	volume={115},
	number={19},
	pages={197202},
	year={2015},
	publisher={APS}
}

@article{xu2015magnetic,
	title={Magnetic structure and crystal-field states of the pyrochlore antiferromagnet Nd 2 Zr 2 O 7},
	author={Xu, J and Anand, VK and Bera, AK and Frontzek, M and Abernathy, Douglas L and Casati, N and Siemensmeyer, K and Lake, B},
	journal={Physical Review B},
	volume={92},
	number={22},
	pages={224430},
	year={2015},
	publisher={APS}
}

@article{benton2016quantum,
	title={Quantum origins of moment fragmentation in Nd 2 Zr 2 O 7},
	author={Benton, Owen},
	journal={Physical Review B},
	volume={94},
	number={10},
	pages={104430},
	year={2016},
	publisher={APS}
}

@article{mydosh1993spin,
	title={Spin Glasses: An Experimental Introduction, Taylor and Francis London},
	author={Mydosh, JA},
	journal={Washington DC},
	year={1993}
}

@article{binder1986spin,
	title={Spin glasses: Experimental facts, theoretical concepts, and open questions},
	author={Binder, Kurt and Young, A Peter},
	journal={Reviews of Modern physics},
	volume={58},
	number={4},
	pages={801},
	year={1986},
	publisher={APS}
}

@article{huang1985some,
	title={Some experimental aspects of spin glasses: A review},
	author={Huang, CY},
	journal={Journal of magnetism and magnetic materials},
	volume={51},
	number={1-3},
	pages={1--74},
	year={1985},
	publisher={Elsevier}
}

@article{matsuhira2001novel,
	title={Novel dynamical magnetic properties in the spin ice compound Dy2Ti2O7},
	author={Matsuhira, K and Hinatsu, Y and Sakakibara, T},
	journal={Journal of Physics: Condensed Matter},
	volume={13},
	number={31},
	pages={L737},
	year={2001},
	publisher={IOP Publishing}
}

@article{jaubert2011magnetic,
	title={Magnetic monopole dynamics in spin ice},
	author={Jaubert, Ludovic DC and Holdsworth, Peter CW},
	journal={Journal of Physics: Condensed Matter},
	volume={23},
	number={16},
	pages={164222},
	year={2011},
	publisher={IOP Publishing}
}

@article{bramwell2009measurement,
	title={Measurement of the charge and current of magnetic monopoles in spin ice},
	author={Bramwell, S Tetal and Giblin, SR and Calder, S and Aldus, R and Prabhakaran, D and Fennell, T},
	journal={Nature},
	volume={461},
	number={7266},
	pages={956--959},
	year={2009},
	publisher={Nature Publishing Group}
}

@article{wannier1950antiferromagnetism,
	title={Antiferromagnetism. the triangular ising net},
	author={Wannier, GH},
	journal={Physical Review},
	volume={79},
	number={2},
	pages={357},
	year={1950},
	publisher={APS}
}

@article{wannier1973errata,
	title={ERRATA: Antiferromagnetism. The Triangular Ising Net},
	author={Wannier, GH},
	journal={Phys. Rev. B},
	volume={7},
	pages={5017},
	year={1973}
}

@article{houtappel1950order,
	title={Order-disorder in hexagonal lattices},
	author={Houtappel, Raymond Marie Ferdinand},
	journal={Physica},
	volume={16},
	number={5},
	pages={425--455},
	year={1950},
	publisher={Elsevier}
}


@article{villain1979insulating,
	title={Insulating spin glasses},
	author={Villain, Jacques},
	journal={Zeitschrift f{\"u}r Physik B Condensed Matter},
	volume={33},
	number={1},
	pages={31--42},
	year={1979},
	publisher={Springer}
}

@article{binder1986spin,
	title={Spin glasses: Experimental facts, theoretical concepts, and open questions},
	author={Binder, Kurt and Young, A Peter},
	journal={Reviews of Modern physics},
	volume={58},
	number={4},
	pages={801},
	year={1986},
	publisher={APS}
}

@article{takatsu2011quantum,
	title={Quantum spin fluctuations in the spin-liquid state of Tb2Ti2O7},
	author={Takatsu, Hiroshi and Kadowaki, Hiroaki and Sato, Taku J and Lynn, Jeffrey W and Tabata, Yoshikazu and Yamazaki, Teruo and Matsuhira, Kazuyuki},
	journal={Journal of Physics: Condensed Matter},
	volume={24},
	number={5},
	pages={052201},
	year={2011},
	publisher={IOP Publishing}
}

@article{singh2012nonconventional,
	title={Nonconventional spin glass transition in a chemically ordered pyrochlore},
	author={Singh, DK and Lee, YS},
	journal={Physical review letters},
	volume={109},
	number={24},
	pages={247201},
	year={2012},
	publisher={APS}
}

@article{gaudet2019quantum,
	title={Quantum spin ice dynamics in the dipole-octupole pyrochlore magnet Ce 2 Zr 2 O 7},
	author={Gaudet, Jonathan and Smith, EM and Dudemaine, J and Beare, J and Buhariwalla, CRC and Butch, Nicholas P and Stone, MB and Kolesnikov, AI and Xu, Guangyong and Yahne, DR and others},
	journal={Physical review letters},
	volume={122},
	number={18},
	pages={187201},
	year={2019},
	publisher={APS}
}

@article{jurvcivsinova2015second,
	title={The second order phase transitions of the spin-1 Ising model on pure Husimi lattices with elementary triangles: Exact results},
	author={Jur{\v{c}}i{\v{s}}inov{\'a}, E and Jur{\v{c}}i{\v{s}}in, M},
	journal={Physics Letters A},
	volume={379},
	number={12-13},
	pages={933--940},
	year={2015},
	publisher={Elsevier}
}

@article{tamura2013second,
	title={Second-order phase transition in the Heisenberg model on a triangular lattice with competing interactions},
	author={Tamura, Ryo and Tanaka, Shu and Kawashima, Naoki},
	journal={Physical Review B},
	volume={87},
	number={21},
	pages={214401},
	year={2013},
	publisher={APS}
}

@article{snyder2004low,
	title={Low-temperature spin freezing in the Dy 2 Ti 2 O 7 spin ice},
	author={Snyder, J and Ueland, BG and Slusky, JS and Karunadasa, H and Cava, Robert Joseph and Schiffer, P},
	journal={Physical Review B},
	volume={69},
	number={6},
	pages={064414},
	year={2004},
	publisher={APS}
}

@article{ehlers2002dynamical,
	title={Dynamical crossover in ‘hot’spin ice},
	author={Ehlers, G and Cornelius, AL and Orendac, M and Kajnakova, M and Fennell, T and Bramwell, ST and Gardner, JS},
	journal={Journal of Physics: Condensed Matter},
	volume={15},
	number={2},
	pages={L9},
	year={2002},
	publisher={IOP Publishing}
}

@article{enjalran2004spin,
	title={The spin liquid state of the Tb2Ti2O7 pyrochlore antiferromagnet: a puzzling state of affairs},
	author={Enjalran, M and Gingras, Michel JP and Kao, YJ and Del Maestro, A and Molavian, HR},
	journal={Journal of Physics: Condensed Matter},
	volume={16},
	number={11},
	pages={S673},
	year={2004},
	publisher={IOP Publishing}
}

@article{greedan1986spin,
	title={Spin-glass-like behavior in Y2Mo2O7, a concentrated, crystalline system with negligible apparent disorder},
	author={Greedan, JE and Sato, M and Yan, Xu and Razavi, FS},
	journal={Solid state communications},
	volume={59},
	number={12},
	pages={895--897},
	year={1986},
	publisher={Elsevier}
}

@article{petrenko2013low,
	title={Low-temperature magnetisation process in the cubic pyrochlore quantum antiferromagnet, Er 2 Ti 2 O 7},
	author={Petrenko, OA and Lees, MR and Balakrishnan, G},
	journal={The European Physical Journal B},
	volume={86},
	number={10},
	pages={416},
	year={2013},
	publisher={Springer}
}
@article{nakatsuji2006metallic,
	title={Metallic spin-liquid behavior of the geometrically frustrated Kondo lattice Pr 2 Ir 2 O 7},
	author={Nakatsuji, S and Machida, Y and Maeno, Y and Tayama, T and Sakakibara, T and Van Duijn, J and Balicas, L and Millican, JN and Macaluso, RT and Chan, Julia Y},
	journal={Physical review letters},
	volume={96},
	number={8},
	pages={087204},
	year={2006},
	publisher={APS}
}
@article{taguchi2003magnetic,
	title={Magnetic Field Induced Sign Reversal of the Anomalous Hall Effect in a Pyrochlore Ferromagnet N d 2 M o 2 O 7: Evidence for a Spin Chirality Mechanism},
	author={Taguchi, Y and Sasaki, T and Awaji, S and Iwasa, Y and Tayama, T and Sakakibara, T and Iguchi, S and Ito, T and Tokura, Y},
	journal={Physical review letters},
	volume={90},
	number={25},
	pages={257202},
	year={2003},
	publisher={APS}
}

@article{jin2001superconductivity,
	title={Superconductivity in the correlated pyrochlore Cd 2 Re 2 O 7},
	author={Jin, R and He, J and McCall, S and Alexander, CS and Drymiotis, F and Mandrus, D},
	journal={Physical Review B},
	volume={64},
	number={18},
	pages={180503},
	year={2001},
	publisher={APS}
}


@article{toews2018disorder,
	title={Disorder dependence of monopole dynamics in Dy 2 Ti 2 O 7 probed via thermal transport measurements},
	author={Toews, WH and Reid, JA and Nadas, RB and Rahemtulla, A and Kycia, S and Munsie, TJS and Dabkowska, HA and Gaulin, BD and Hill, RW},
	journal={Physical Review B},
	volume={98},
	number={13},
	pages={134446},
	year={2018},
	publisher={APS}
}

@article{castelnovo2008magnetic,
	title={Magnetic monopoles in spin ice},
	author={Castelnovo, Claudio and Moessner, Roderich and Sondhi, Shivaji L},
	journal={Nature},
	volume={451},
	number={7174},
	pages={42--45},
	year={2008},
	publisher={Nature Publishing Group}
}

@article{morris2009dirac,
	title={Dirac strings and magnetic monopoles in the spin ice Dy2Ti2O7},
	author={Morris, David Jonathan Pryce and Tennant, DA and Grigera, SA and Klemke, B and Castelnovo, C and Moessner, R and Czternasty, C and Meissner, M and Rule, KC and Hoffmann, J-U and others},
	journal={Science},
	volume={326},
	number={5951},
	pages={411--414},
	year={2009},
	publisher={American Association for the Advancement of Science}
}

@article{jaubert2011magnetic,
	title={Magnetic monopole dynamics in spin ice},
	author={Jaubert, Ludovic DC and Holdsworth, Peter CW},
	journal={Journal of Physics: Condensed Matter},
	volume={23},
	number={16},
	pages={164222},
	year={2011},
	publisher={IOP Publishing}
}

@article{fennell2009magnetic,
	title={Magnetic Coulomb phase in the spin ice Ho2Ti2O7},
	author={Fennell, Tom and Deen, PP and Wildes, AR and Schmalzl, K and Prabhakaran, D and Boothroyd, AT and Aldus, RJ and McMorrow, DF and Bramwell, ST},
	journal={Science},
	volume={326},
	number={5951},
	pages={415--417},
	year={2009},
	publisher={American Association for the Advancement of Science}
}

@article{devi2020emergence,
	title={Emergence of weak pyrochlore phase and signature of field induced spin ice ground state in Dy2- xLaxZr2O7; x= 0, 0.15, 0.3},
	author={Devi, Sheetal and Ali, Anzar and Rajput, Sarita and Singh, Yogesh and Maitra, Tulika and Yadav, CS},
	journal={Journal of Physics: Condensed Matter},
	volume={32},
	number={36},
	pages={365804},
	year={2020},
	publisher={IOP Publishing}
}
@article{bramwell2001spin,
	title={Spin correlations in Ho 2 Ti 2 O 7: a dipolar spin ice system},
	author={Bramwell, ST and Harris, MJ and Den Hertog, BC and Gingras, MJP and Gardner, JS and McMorrow, DF and Wildes, AR and Cornelius, AL and Champion, JDM and Melko, RG and others},
	journal={Physical Review Letters},
	volume={87},
	number={4},
	pages={047205},
	year={2001},
	publisher={APS}
}

@article{siddharthan1999ising,
	title={Ising pyrochlore magnets: Low-temperature properties,“ice rules,” and beyond},
	author={Siddharthan, R and Shastry, BS and Ramirez, AP and Hayashi, A and Cava, Robert Joseph and Rosenkranz, S},
	journal={Physical review letters},
	volume={83},
	number={9},
	pages={1854},
	year={1999},
	publisher={APS}
}

@article{fukazawa2002magnetic,
	title={Magnetic anisotropy of the spin-ice compound Dy 2 Ti 2 O 7},
	author={Fukazawa, H and Melko, RG and Higashinaka, R and Maeno, Y and Gingras, MJP},
	journal={Physical Review B},
	volume={65},
	number={5},
	pages={054410},
	year={2002},
	publisher={APS}
}

@article{dupuis2002aging,
	title={Aging and memory properties of topologically frustrated magnets},
	author={Dupuis, V and Vincent, E and Hammann, J and Greedan, JE and Wills, AS},
	journal={Journal of applied physics},
	volume={91},
	number={10},
	pages={8384--8386},
	year={2002},
	publisher={American Institute of Physics}
}

==> RefS.tex <==
@article{devi2020emergence,
	title={Emergence of weak pyrochlore phase and signature of field induced spin ice ground state in Dy 2- x La x Zr 2 O 7; x= 0, 0.15, 0.3},
	author={Devi, Sheetal and Ali, Anzar and Rajput, Sarita and Singh, Yogesh and Maitra, Tulika and Yadav, CS},
	journal={Journal of Physics: Condensed Matter},
	volume={32},
	pages={365804},
	year={2020},
	publisher={IOP Publishing}
}

@article{ramon2019absence,
	title={Absence of spin-ice state in the disordered fluorite D y 2 Z r 2 O 7},
	author={Ramon, Jonathan Gustavo Acosta and Wang, CW and Ishida, L and Bernardo, PL and Leite, MM and Vichi, Fl{\'a}vio Maron and Gardner, JS and Freitas, RS},
	journal={Physical Review B},
	volume={99},
	number={21},
	pages={214442},
	year={2019},
	publisher={APS}
}
